Adversarial Distortion for Learned Video Compression

In this paper, we present a novel adversarial lossy video compression model. At extremely low bit-rates, standard video coding schemes suffer from unpleasant reconstruction artifacts such as blocking, ringing etc. Existing learned neural approaches to video compression have achieved reasonable success on reducing the bit-rate for efficient transmission and reduce the impact of artifacts to an extent. However, they still tend to produce blurred results under extreme compression. In this paper, we present a deep adversarial learned video compression model that minimizes an auxiliary adversarial distortion objective. We find this adversarial objective to correlate better with human perceptual quality judgement relative to traditional quality metrics such as MS-SSIM and PSNR. Our experiments using a state-of-the-art learned video compression system demonstrate a reduction of perceptual artifacts and reconstruction of detail lost especially under extremely high compression.

==> related_work.tex <==
\textbf{Learned video compression} There have been several proposed approaches to apply deep learning to the problem of lossy video compression, among which we find our work to be particularly relevant to those that are based on encoder-decoder modeling in the variational framework. 

Our work is most relevant to \cite{habibian2019video} which performs video compression using a 3d autoencoder and an autoregressive prior based on Pixel-CNNs\cite{van2016conditional} over a discrete latent space. This model achieves state-of-the-art results in reconstruction quality at various compression levels. Another relevant autoencoder based video compression model, \cite{han2018deep} is jointly trained to transform videos into a low-dimensional latent representation and to decorrelate the latents through model-based entropy coding. While the above two approaches do not suffer from the artifacts produced by traditional coding schemes that employ blocking, they minimize their distortion error measured using either $l_1$ norm or $l_2$ norm; this raises the possibility of the decoded output suffering from blurring and unrealistic texture issues, degrading the perceptual quality after compression.

Among other approaches to tackle video compression using neural networks are those that utilize block-prediction and frame-prediction from spatio-temporal contextual information to learn compressible video representations\cite{chen2019learning, chen2017deepcoder}. \cite{lu2019dvc} propose an end-to-end trainable autoencoder based video compression model which utilizes learned neural networks to perform motion estimation and residual prediction. \cite{djelouah2019neural} is a similar deep-learning based video compression model that performs optical flow-based motion compensation in the pixel space, and residual prediction in the latent space. However, since these above approaches still operate via block-prediction within frames like conventional video coding schemes, they are also prone to the same artifacts that plague conventional video-coding schemes (blurring, blocking, ringing etc.).

\textbf{Generative adversarial networks}
The crux of our work is based on the impressive feat achieved by Generative Adversarial Networks in producing increasingly realistic natural images and videos \cite{karras2019style,karras2017progressive,zhang2018self,brock2018large,clark2019efficient}, we find this as suggestive of the objective function they optimize to reflect image/video realness as perceived by humans. In this direction of incorporating GANs into lossy compression systems, \cite{agustsson2019generative} have successfully added an auxiliary adversarial component to their lossy image compression system that results in superior image compression with reduced perceptual artifacts. However, there is little work involving the application of adversarial components to lossy video compression systems due to scaling issues; this is also why we believe the resolution of video-generating GANs have lagged behind that of image-generating GANs. We have found success in tackling this scaling issue via factorization of our adversarial discriminator into smaller neural network components and show results that demonstrate our compression system's relatively improved perceptual quality even under extreme compression.
